BRExIt: On Opponent Modelling in Expert Iteration

Finding a best response policy is a central objective in game theory and multi-agent learning, with modern population-based training approaches employing reinforcement learning algorithms as best-response oracles to improve play against candidate opponents (typically previously learnt policies). We propose Best Response Expert Iteration (BRExIt), which accelerates learning in games by incorporating opponent models into the state-of-the-art learning algorithm Expert Iteration (ExIt). BRExIt aims to (1) improve feature shaping in the apprentice, with a policy head predicting opponent policies as an auxiliary task, and (2) bias opponent moves in planning towards the given or learnt opponent model, to generate apprentice targets that better approximate a best response. In an empirical ablation on BRExIt's algorithmic variants against a set of fixed test agents, we provide statistical evidence that BRExIt learns better performing policies than ExIt.

==> sections/algorithms/expert_iteration_apprentice_update_simultaneous.tex <==
\begin{algorithm}
\KwIn{\textit{Neural net with 3 head types}: $NN = (\pi_{\bm{\theta}}, \textcolor{orange}{\hat{\bm{\pi}}^{\bm{\psi}}_{-i}}, V_{\bm{\phi}})$}
\KwIn{\textit{Dataset}: $D$}
\For{$t = 0, 1, 2, \dots$} {

   Sample batch of size $n$: $(s_t, \pi_{MCTS}(s_t), \textcolor{orange}{\bm{\pi_{-i}}(s_t)}, v)_{1, \ldots, n} \sim D$\;

   MSE value loss: $\mathcal{L}_{v} = (v - V_{\bm{\phi}}(s_t))^2$

   CE policy loss $\mathcal{L}_{\pi} = \pi_{MCTS}(s_t) \log{(\pi_{\bm{\theta}}(s_t))}$ \;

   \textcolor{orange}{CE policy inference loss: $\mathcal{L}_{PI} = \frac{1}{|\bm{\pi}_{-i}|} \bm{\pi}_{-i}(s_t) \log{(\hat{\bm{\pi^{\psi}}}_{-i}(s_t))}$ } \;

   \textcolor{orange}{Policy inference weight: $\lambda = \frac{1}{\sqrt{\mathcal{L}_{PI}}}$}\;

   Compute weighted sum of losses $\mathcal{L}_{total} = \textcolor{orange}{\lambda} (\mathcal{L}_{v} + \mathcal{L}_{\pi}) + \textcolor{orange}{\mathcal{L}_{PI}}$ \;

   Backpropagate gradients $\nabla\mathcal{L}_{total}$ to update $\bm{\theta}, \textcolor{orange}{\bm{\psi}}, \bm{\phi}$ \;

}

\caption{BRExIt model update (Simultaneous game)}\label{algorithm:brexit_update_simultaneous}
\end{algorithm}


==> sections/algorithms/expert_iteration_data_collection_simultaneous.tex <==
\begin{algorithm}
    \KwIn{\textit{NN being trained}: $NN = (\text{apprentice } \pi, \textcolor{orange}{\text{opponent models } \hat{\bm{\pi}}_{-i}}, \text{critic } V)$}
    \KwIn{\textcolor{orange}{\textit{Opponent policies}: $\bm{\pi_{-i}}$}}
    \KwIn{Environment: $E = (\mathcal{P}, \rho_0)$}
    Initialize dataset: $D = [\ ]$\;
    Sample initial state $s_0 \sim \rho_0$\;
    \For{$t = 0, 1, 2, \dots$} {
       Search using apprentice and opponent models: $a_t, tree_t = MCTS(\pi, \textcolor{orange}{\bm{\pi_{-i}}}, V)$\;
       Derive from $tree$: $\forall a \in \mathcal A\; \pi_{MCTS}(s_t, a) = \frac{N_{root}(s_t, a)}{\sum_{a'} N_{root}(s_t, a')}$\;
       Act in the game: $s_{t+1}, \bm{r}_t \sim \mathcal{P}(s_t, ([a_t] \cup [a^t_j \sim \pi_j(s_t) \quad \forall \pi_j \in \bm{\pi_{-i}}])$\;
       Add datapoint: $D = D \cup (s_t, \bm{r}^i_t, \pi_{MCTS}(s_t, \cdot), \textcolor{orange}{\bm{\pi_{-i}}(s_t)} )$\;
    }
    \KwReturn $D$\;

    \caption{BRExIt single match data collection (Simultaneous game).}
    \label{algorithm:brexit_collection_simultaneous}
\end{algorithm}


==> sections/training_setup.tex <==
\input{sections/algorithms/expert_iteration_data_collection.tex}
\input{sections/algorithms/expert_iteration_apprentice_update.tex}
\input{sections/algorithms/expert_iteration_training_loop.tex}

\subsection{Domain}

\subsection{Evaluation metrics}

Things to look out for
\begin{itemize}
\item Does Opponent modelling perform better when its opponent model is trained
by (1) observing single actions from the opponent or (2) observing the full
distribution over actions (exploiting perfect opponent model).

\item Does BRExIt perform online adaptation.
\end{itemize}

\subsubsection{Evaluating online adaptation}

As inspired from~\cite{al2017continuous}. Online adaptation can be viewed as a
\textbf{few-shot} learning problem, where a \textit{fixed} and already trained
agent $\pi_{\theta}$ has to learn to compute a best response towards agent
$\pi^{other}$ with a limited amount of interaction (A few episodes, a few
actions).

\paragraph{Generating test policies:}

A set of increasingly better / different policies are pre-computed in advance. These policies can be the policies trained via algorithm X under (naive) self-play for a fixed number of episodes. During training, a few checkpoints of these policies are frozen to serve as testing policies. These test policies can be regarded as a curricula of tasks, pre-determined at testing time, but unknown to the agent being tested.

\paragraph{Testing against test policies:}

We run our trained agent(s) against the policy snapshots described above. We let our trained agent(s) play X episodes against each fixed policy before the test policy changes to a different one. Note: internal RNN states are zeroed on every episode termination.
 
% ~\cite{mnih2013playing} introduced the Deep Q Network algorithm and neural network architecture, a deep variant of Q Learning~\cite{Watkins1989}. Many incremental
 


Nash equilibria (of meta strategies) are difficult to learn. They might have a
lot of structure though, which we exploit via opponent modelling.

Multiagent algorithms that generate game-playing agents have achieved good
performance by computing best responses to local Nash equilibria. However,
playing according to Nash equilibria misses the opportunity to adapt / exploit
suboptimal policies that may be encountered during play. i.e How to perform
online adaptation to opponents.

